A Framework for Complementary Companion Character Behavior in Video Games

We propose a game development framework capable of governing the behavior of complementary companions in a video game. A "complementary" action is contrasted with a mimicking action and is defined as any action by a friendly non-player character that furthers the player's strategy. This is determined through a combination of both player action and game state prediction processes while allowing the AI companion to experiment. We determine the location of interest for companion actions based on a dynamic set of regions customized to the individual player. A user study shows promising results; a majority of participants familiar with game design react positively to the companion behavior, stating that they would consider using the frame-work in future games themselves.

==> sections/flowchart.tex <==
\begin{figure*}
  \centerline{
    \includegraphics[width=0.9\textwidth]{figures/flowchart/full.jpg}
  }
  \label{fig:flowchart}
  \caption{A visualization of the companion's decision-making process}
\end{figure*}
